Controlling Vocabulary, Syntax, and Length in Image Descriptions

Adapting text to readers' knowledge and purposes requires identifying linguistic demands and generating text that meets them. We study the generation step, taking vocabulary, syntax, and length targets as given: an image description may need to retain necessary terms while using short, simple sentences. Motivated by future on-device use, we distill a 125B teacher's generated descriptions into Qwen3-VL vision-language models (VLMs) with 4B, 8B, and 32B parameters. We filter teacher outputs by linguistic rules and train students on retained text using supervised fine-tuning (SFT), then apply direct preference optimization (DPO) to pairs generated by each student. We compare these training stages with prompting across eight target combinations. Automatic evaluation uses two sets of 100 images excluded from task-specific training, plus a third set of 100 images frozen before generation; our primary metric requires the exact requested word ranges. Averaged across the first two sets, 4B strict joint success rises from 21.8% with prompting to 47.7% with SFT+DPO. Students at all sizes improve over prompting on both image sets, and a blinded human study finds no detectable loss in rated faithfulness or naturalness after training. These results show that training on filtered teacher-generated text, followed by preference optimization, improves how often an image description meets vocabulary, syntax, and length requirements together.

==> tables/main_results.tex <==
\begin{tabular}{llccccc}
\toprule
Size & Method & Format & Length & Vocabulary & Syntax & All \\
\midrule
4B & Prompt only & 99.4 \ci{98.5}{100.0} & 87.2 \ci{84.8}{89.6} & 60.1 \ci{57.0}{63.2} & 74.4 \ci{71.5}{77.2} & 36.0 \ci{33.0}{39.1} \\
 & SFT & 99.4 \ci{98.6}{99.9} & 91.4 \ci{89.5}{93.1} & 60.8 \ci{57.5}{64.0} & 82.6 \ci{80.0}{85.2} & 44.9 \ci{41.2}{48.4} \\
 & SFT+DPO (orig.) & 99.6 \ci{99.1}{100.0} & 91.0 \ci{88.9}{92.9} & 60.9 \ci{57.4}{64.1} & 93.1 \ci{91.1}{95.0} & 51.0 \ci{47.2}{54.5} \\
 & SFT+DPO & 99.6 \ci{99.1}{100.0} & 90.4 \ci{88.4}{92.1} & 63.6 \ci{60.1}{67.2} & 93.9 \ci{91.9}{95.8} & 53.8 \ci{50.1}{57.4} \\
\midrule
8B & Prompt only & 98.8 \ci{97.1}{99.8} & 76.6 \ci{73.9}{79.1} & 55.2 \ci{52.4}{58.0} & 92.0 \ci{89.6}{94.0} & 38.6 \ci{35.9}{41.4} \\
 & SFT & 99.2 \ci{97.6}{100.0} & 95.0 \ci{93.1}{96.8} & 62.5 \ci{59.4}{65.9} & 87.5 \ci{84.9}{90.0} & 50.5 \ci{46.9}{54.1} \\
 & SFT+DPO (orig.) & 99.4 \ci{98.1}{100.0} & 86.0 \ci{83.5}{88.8} & 66.4 \ci{63.2}{69.6} & 95.1 \ci{93.0}{96.9} & 54.5 \ci{51.0}{58.2} \\
 & SFT+DPO & 99.1 \ci{97.5}{100.0} & 92.6 \ci{90.5}{94.8} & 70.4 \ci{67.4}{73.2} & 95.2 \ci{93.2}{97.0} & 61.1 \ci{57.6}{64.8} \\
\midrule
32B & Prompt only & 99.4 \ci{98.8}{99.9} & 53.1 \ci{48.9}{56.9} & 57.6 \ci{54.2}{61.0} & 95.1 \ci{93.1}{97.0} & 31.8 \ci{27.9}{35.5} \\
 & SFT & 99.9 \ci{99.6}{100.0} & 96.0 \ci{94.4}{97.5} & 63.9 \ci{60.9}{67.0} & 90.1 \ci{87.6}{92.4} & 54.5 \ci{51.2}{58.0} \\
 & SFT+DPO (orig.) & 99.5 \ci{99.0}{99.9} & 86.2 \ci{83.2}{88.9} & 66.5 \ci{63.1}{70.1} & 95.6 \ci{93.9}{97.2} & 55.0 \ci{51.1}{58.9} \\
 & SFT+DPO & 99.4 \ci{98.6}{99.9} & 97.4 \ci{96.1}{98.5} & 65.9 \ci{62.9}{69.1} & 96.5 \ci{94.9}{98.0} & 61.5 \ci{58.1}{65.1} \\
\bottomrule
\end{tabular}


==> tables/per_condition.tex <==
\begin{tabular}{@{}lcccccccccccc@{}}
\toprule
Condition & \multicolumn{4}{c}{4B} & \multicolumn{4}{c}{8B} & \multicolumn{4}{c}{32B} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
(vocabulary, syntax, length) & P & S & O & D & P & S & O & D & P & S & O & D \\
\midrule
basic, simple, short & 81 & 84 & 78 & 82 & 82 & 83 & 74 & 76 & 61 & 78 & 76 & 78 \\
basic, simple, long & 41 & 53 & 63 & 57 & 34 & 62 & 71 & 69 & 61 & 68 & 65 & 74 \\
basic, complex, short & 19 & 32 & 51 & 59 & 51 & 39 & 62 & 67 & 23 & 58 & 52 & 67 \\
basic, complex, long & 43 & 60 & 67 & 75 & 67 & 65 & 66 & 74 & 47 & 63 & 67 & 85 \\
advanced, simple, short & 28 & 33 & 34 & 39 & 18 & 32 & 38 & 43 & 18 & 40 & 45 & 43 \\
advanced, simple, long & 24 & 26 & 34 & 32 & 10 & 38 & 41 & 51 & 24 & 40 & 43 & 42 \\
advanced, complex, short & 14 & 29 & 34 & 39 & 17 & 36 & 40 & 50 & 5 & 33 & 36 & 45 \\
advanced, complex, long & 38 & 42 & 47 & 47 & 30 & 49 & 44 & 59 & 15 & 56 & 56 & 58 \\
\midrule
All conditions & 36.0 & 44.9 & 51.0 & 53.8 & 38.6 & 50.5 & 54.5 & 61.1 & 31.8 & 54.5 & 55.0 & 61.5 \\
\bottomrule
\end{tabular}


==> tables/test2_results.tex <==
\begin{tabular}{llcccc}
\toprule
& & \multicolumn{2}{c}{Strict length rule} & \multicolumn{2}{c}{Within 2 words} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
Size & Method & Length & All & Length & All \\
\midrule
4B & Prompt only & 57.8 \ci{54.6}{61.3} & 20.9 \ci{18.2}{23.8} & 86.1 \ci{84.0}{88.4} & 35.4 \ci{32.0}{38.9} \\
 & SFT & 63.1 \ci{59.9}{66.4} & 29.9 \ci{27.1}{32.8} & 89.2 \ci{87.2}{91.1} & 43.2 \ci{39.8}{46.6} \\
 & SFT+DPO (orig.) & 62.4 \ci{59.1}{65.5} & 37.0 \ci{33.8}{40.2} & 90.5 \ci{88.0}{92.8} & 52.8 \ci{49.4}{56.1} \\
 & SFT+DPO & 67.0 \ci{63.9}{70.0} & 38.8 \ci{35.5}{42.0} & 91.9 \ci{89.9}{93.8} & 52.9 \ci{49.4}{56.5} \\
\midrule
8B & Prompt only & 51.0 \ci{47.9}{54.1} & 25.6 \ci{22.8}{28.5} & 79.2 \ci{76.6}{82.0} & 38.0 \ci{34.9}{41.4} \\
 & SFT & 72.8 \ci{70.1}{75.4} & 33.0 \ci{29.6}{36.6} & 95.1 \ci{93.5}{96.6} & 45.4 \ci{42.2}{48.9} \\
 & SFT+DPO (orig.) & 60.4 \ci{56.2}{64.2} & 33.6 \ci{30.2}{37.0} & 86.8 \ci{84.4}{89.0} & 49.0 \ci{45.6}{52.3} \\
 & SFT+DPO & 72.9 \ci{69.2}{76.4} & 41.8 \ci{38.1}{45.5} & 93.6 \ci{91.9}{95.1} & 55.0 \ci{51.5}{58.5} \\
\midrule
32B & Prompt only & 29.9 \ci{26.1}{33.9} & 17.6 \ci{15.0}{20.5} & 55.0 \ci{50.7}{59.2} & 32.8 \ci{29.4}{36.2} \\
 & SFT & 70.6 \ci{67.1}{74.3} & 36.6 \ci{33.1}{40.2} & 95.2 \ci{93.5}{96.8} & 50.1 \ci{46.7}{53.8} \\
 & SFT+DPO (orig.) & 58.2 \ci{54.4}{62.3} & 33.8 \ci{30.6}{37.1} & 87.0 \ci{84.2}{89.8} & 51.2 \ci{47.8}{54.9} \\
 & SFT+DPO & 77.2 \ci{74.4}{80.2} & 46.9 \ci{43.5}{50.5} & 96.2 \ci{94.5}{97.8} & 59.2 \ci{55.9}{62.6} \\
\bottomrule
\end{tabular}

